Joint Convexity of Error Probability in Blocklength and Transmit Power in the Finite Blocklength Regime

To support ultra-reliable and low-latency services for mission-critical applications, transmissions are usually carried via short blocklength codes, i.e., in the so-called finite blocklength (FBL) regime. Different from the infinite blocklength regime where transmissions are assumed to be arbitrarily reliable at the Shannon's capacity, the reliability and capacity performances of an FBL transmission are impacted by the coding blocklength. The relationship among reliability, coding rate, blocklength and channel quality has recently been characterized in the literature, considering the FBL performance model. In this paper, we follow this model, and prove the joint convexity of the FBL error probability with respect to blocklength and transmit power within a region of interest, as a key enabler for designing systems to achieve globally optimal performance levels. Moreover, we apply the joint convexity to general use cases and efficiently solve the joint optimization problem in the setting with multiple users. We also extend the applicability of the proposed approach by proving that the joint convexity still holds in fading channels, as well as in relaying networks. Via simulations, we validate our analytical results and demonstrate the advantage of leveraging the joint convexity compared to other commonly-applied approaches.

==> archive.tex <==

Although the objective function is jointly convex in $\mathbf{m}$ and $\mathbf{p}$ according to Lemma~\ref{lemma:joint_convex}, the constraint~\eqref{con:energy_nonconvex} is still non-convex. We first discuss two approaches partially leveraging the convex feature to solve the joint optimization problem.

{\color{red} swap partially convex and jointly convex}
\subsection{Approaches Based on Partially Convex Feature}
\subsubsection{Integer convex optimization}
Since blocklength ${m_i}$ is an integer variable and total available blocklength is limited , the original problem~\eqref{problem_downlink} can be decomposed into  $\frac{(M-1)!}{(M-N)!}$ sub-problems with fixed $\mathbf{m}=\mathbf{m}^o$ where $\mathbf{m}^o$ is the element in the set of possible blocklength allocation combination $\mathcal{M}$, i.e.,
    \begin{mini!}[2]
    {\mathbf{p}}{\max_i\{\varepsilon_{i}\}}
    {\label{problem_int}}{}
    \addConstraint{\mathbf{m}}{= \mathbf{m}^o}
    \addConstraint{\sum^N_im_ip_i}{\leq E}
    \label{con:decoposed_E}
    \addConstraint{\varepsilon_i}{\leq \varepsilon_{\max}, \gamma_i\geq 1, \forall i=1,...,N}
    \end{mini!}
    As we proven in Lemma~\ref{lemma:joint_convex}, $\varepsilon_i$ is convex in $\mathbf{p}$ and the rest of constraints are either affine or convex %(note that Lemma~\ref{lemma:joint_convex_reformulated} is not necessary for such problem due to fixed $\mathbf{m}^o$). 
    Therefore, the original problem becomes essentially an integer convex optimization problem. In other word, the global optimal solution can be found by comparing the solutions of each decomposed sub-problem with all possible $\mathbf{m}^o$ in $\mathcal{M}$, resulting a computational complexity $\mathcal{O}(\frac{(M-1)!}{(M-N)!}N^2)$. The major drawback of this approach is the complexity, which increases exponentially with the available blocklength and number of UEs. This is especially unpreferred for the future low-latency IoT network connected with possibly massive devices. 
\subsubsection{Iterative searching}
Analog to fixing $\mathbf{m}$, we can also decompose original problem by fixing $\mathbf{p}=\mathbf{p}^o$, i.e.,
        \begin{mini!}[2]
    {\mathbf{m}}{\max_i\{\varepsilon_{i}\}}
    {\label{problem_int2}}{}
    \addConstraint{\mathbf{p}}{= \mathbf{p}^o}
    \addConstraint{\sum^N_im_ip_i}{\leq E}
    \addConstraint{\varepsilon_i}{\leq \varepsilon_{\max}, \gamma_i\geq 1, \forall i=1,...,N}.
    \end{mini!}
    Since both sub-problems~\eqref{problem_int} and~\eqref{problem_int2} are convex, we can solve them alternatively. In particular, for each iteration $k$, we fix $\mathbf{p}=\mathbf{p}^{(k-1)}$ and obtain $\mathbf{m}^{(k)}$ by solve Problem~\ref{problem_int} optimally. Then, we fix $\mathbf{m}=\mathbf{m}^{(k)}$ and obtain $\mathbf{p}^{(k)}$ by solve Problem~\ref{problem_int2} optimally. Specially, $\mathbf{p}^{(0)}$ is an initial value for the first iteration. We repeat above iteration until it converges, where the converge rate  is linear with a computational complexity $\mathcal{O}(2N^2)$~\cite{Tseng_BCD}. The advantage of iterative searching is the low complexity comparing to the integer convex programming. However, the obtained solution of such method is only sub-optimal and highly depends on the initial value.  To improve the performance, one can  redo the algorithm multiple times with randomly choose the initial values. However,  it also increases the overall complexity and still cannot guarantee the global optimum. Furthermore, the cost also increases when the number of user $N$ increases due to the larger random space for the initial value.
\begin{table*}[t]
\centering
 \begin{tabular}{||c| c| c| c|c||} 
 \hline
& Convexity & Optimum & Complexity & Scalability \\ 
 \hline
 integer convex optimization & partial &\cellcolor{green!25} global optimal & high & bad \\ 
 \hline
 iterative search & partial & sub-optimal & \cellcolor{green!25} low & decent \\
 \hline
 jointly convex optimization & joint &\cellcolor{green!25}  global optimal &\cellcolor{green!25}  low &\cellcolor{green!25}  good \\
 \hline
\end{tabular}
\caption{Properties of integer convex optimization, iterative search and jointly convex optimization. Green color indicates the best quality of the property.}
\label{tab:compare}
\end{table*}
\subsection{Solution based on Joint Convex Feature}
Since both above approaches have certain disadvantage, we are interested in how to turn Problem~\eqref{con:energy_nonconvex} into a jointly convex problem, i.e., reformulating constraint~\eqref{con:total_E_non_convex} to be convex while maintaining the convexity of $\varepsilon_i$. To address this issue, we let $m_i=\frac{1}{a_i}$ and $p_i=b^2_i$, for $i\in \mathcal{N}$. Therefore, we can reformulate problem~\eqref{problem_downlink} with new variables $\mathbf{b}$ and $\mathbf{a}$ as follows 
\begin{mini!}[2]
{\mathbf{a},\mathbf{b}}{\max_{i\in\mathcal{N}}\{\varepsilon_{i}\}}
{\label{problem_downlink_reformulated}}{}
\addConstraint{\sum^N_{i=1}\frac{1}{a_i}}{\leq M}
\addConstraint{\sum^N_{i=1} \frac{b^2_i}{a_i}}{\leq E}
\label{con:energy_nonconvex_reformulated}
\addConstraint{\varepsilon_1\leq\varepsilon_{\max},}{\ \varepsilon_2\leq \varepsilon_{\max}}
\addConstraint{\gamma_1\geq1,}{\ \gamma_2\geq1.}
\end{mini!}

It is trivial to prove the convexity of  reformulated constraint~\eqref{con:energy_nonconvex_reformulated}, since it is the sum of $N$ convex functions. We focus on the convexity of $\varepsilon_i$. Due to the substitution of variables, Lemma~\ref{lemma:joint_convex} is no longer sufficient to prove the convexity. Therefore, we exploit the following lemma to characterizing the problem.
\begin{theorem}
\label{lemma:joint_convex_reformulated}
The problem~\eqref{problem_downlink_reformulated} is jointly convex in $\mathbf{a}$ and $\mathbf{b}$.
\end{theorem}
According to Lemma~\ref{lemma:joint_convex_reformulated}, problem~\eqref{problem_downlink_reformulated} is a convex problem and  can be solved efficiently by standard convex programming methods. It is worth to mention that the problem can also be extended to multi-user scenario with $\mathbf{m}=\{m_i,\forall i=1,...,N\}$ and $\mathbf{p}=\{p_i,\forall i=1,...,N\}$ while the convex feature remains. Moreover, the advantage of this characterization is enable to provide the optimal solution with low complexity of $\mathcal{O}(4N^2)$ while guaranteeing the global optimum, which is also scalable to support low-latency IoT network with massive devices. As a comparison, we show the properties of all three approaches in terms of optimum, complexity and scalability in Table~\ref{tab:compare}.

Although we consider the maximal error probability as our objective function, it should be point out that Lemma~\ref{lemma:joint_convex_reformulated} and Lemma~\ref{lemma:joint_convex_reformulated} can also be applied with other objectives. For instance, we can also take total energy consumption, i.e.,$\sum^N_{i=1}m_i p_i$,  or effective throughput, i.e., $\sum^N_{i=1} D_i(1-\varepsilon_i)$, as the objective function. However, the exact design of the metric for the resource allocation problem is out the main scope of this paper.
